Symbolic Regression via Control Variable Genetic Programming

Learning symbolic expressions directly from experiment data is a vital step in AI-driven scientific discovery. Nevertheless, state-of-the-art approaches are limited to learning simple expressions. Regressing expressions involving many independent variables still remain out of reach. Motivated by the control variable experiments widely utilized in science, we propose Control Variable Genetic Programming (CVGP) for symbolic regression over many independent variables. CVGP expedites symbolic expression discovery via customized experiment design, rather than learning from a fixed dataset collected a priori. CVGP starts by fitting simple expressions involving a small set of independent variables using genetic programming, under controlled experiments where other variables are held as constants. It then extends expressions learned in previous generations by adding new independent variables, using new control variable experiments in which these variables are allowed to vary. Theoretically, we show CVGP as an incremental building approach can yield an exponential reduction in the search space when learning a class of expressions. Experimentally, CVGP outperforms several baselines in learning symbolic expressions involving multiple independent variables.

==> tex/10-proof.tex <==
\section{Proof of Lemma~\ref{lem:searchspace}} \label{sec:apx-proof}
\begin{proof}
    Because all operands are binary, a symbolic expression tree of $l$ nodes has $\frac{l+1}{2}$ leaves and $\frac{l-1}{2}$ internal nodes. 
    %
    The number of binary trees of $\frac{l-1}{2}$ internal nodes is given by the Cantalan number $C_{{(l-1)}/{2}} = \frac{l-1}{{l+1}}{l-1 \choose {(l-1)}/{2}}$, which asymptotically scales at $\frac{2^{{l-1}}}{{(\frac{l-1}{2})}^{3/2}\sqrt{\pi}}$. 
    %
    A symbolic expression replaces each internal node of a binary tree with an operand and replaces each leaf with either a constant or one of the input variables. 
    %
    Because there are $o$ operands and $m$ input variables, the total number of different symbolic expression trees involving $l$ nodes is given by:
    \begin{align}
    A(l) = C_{(l-1)/{2}} (m+1)^{\frac{l+1}{2}} o^\frac{l-1}{2}
    &=\frac{{l-1}}{{l+1}}{l-1 \choose {(l-1)}/{2}}(m+1)^{\frac{l+1}{2}} o^\frac{l-1}{2} \nonumber\\
    &\sim \frac{(4(m+1)o)^{\frac{l-1}{2}}}{ \left(\frac{l-1}{2}\right)^{3/2}}.
    \end{align}
    Hence, the total number of trees up to $l$ nodes is:
    \begin{align}
    S(l) = \sum_{i=0}^{(l-1)/2} A(2i+1) \sim \sum_{i=0}^{(l-1)/2} \frac{(4(m+1)o)^{i}}{ i^{3/2}}.
    \end{align}
    When $i$ is sufficiently large,
    \begin{align}
    (4(m+1)o)^{i/2} \leq \frac{(4(m+1)o)^{i}}{ i^{3/2}} \leq (4(m+1)o)^{i}.
    \end{align}
    Therefore, $$S(l) \leq \sum_{i=0}^{(l-1)/2} (4(m+1)o)^{i} \in \mathcal{O}((4(m+1)o)^{(l-1)/2}),$$ and
    $$S(l) \geq (4(m+1)o)^{(l-1)/2} / ((l-1)/2)^{3/2} \geq (4(m+1)o)^{(l-1)/4},$$ which implies 
    $$S(l) \in \Omega((4(m+1)o)^{\frac{l-1}{4}}).$$
\end{proof}
